Reversible Computations of One-Way Counter Automata

Deterministic one-way time-bounded multi-counter automata are studied with respect to their ability to perform reversible computations, which means that the automata are also backward deterministic and, thus, are able to uniquely step the computation back and forth. We study the computational capacity of such devices and obtain separation results between irreversible and reversible k-counter automata for superpolynomial time. For exponential time we obtain moreover an infinite and tight hierarchy with respect to the number of counters. This hierarchy is shown with Kolmogorov complexity and incompressibility arguments. In this way, on passing we can prove this hierarchy also for ordinary counter automata. This improves the known hierarchy for ordinary counter automata in the sense that here we consider a weaker acceptance condition. Then, it turns out that k+1 reversible counters are not better than k ordinary counters and vice versa. Finally, almost all usually studied decidability questions turn out to be undecidable and not even semidecidable for reversible multi-counter automata, if at least two counters are provided.

==> eptcsdata.tex <==
\providecommand{\firstpage}{126}
\providecommand{\publicationstatus}{H. Bordihn, G. Horv\'ath, G. Vaszil (Eds.): 12th International Workshop on\\Non-Classical Models of Automata and Applications (NCMA 2022)\\
EPTCS 367, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.367.9}{10.4204/EPTCS.367.9}}
\pdfoutput=1

